Extricating IoT Devices from Vendor Infrastructure with Karl

Most consumer IoT devices are vertically integrated with cloud-side infrastructure. Such architectures present enormous risk to user data, exacerbated by vendor heterogeneity and the inability for users to audit cloud-side activity. A more promising approach would be to leverage local hardware, providing users control over how their data is processed and why it can be shared with other devices or the Internet. Karl is a new smart-home framework designed to host IoT computation and storage on user-chosen devices. A key insight in Karl's modular programming model is that a familiar interface (inspired by serverless) can capture most modern cloud-side IoT components under a single framework, which executes modules agnostic of hardware location. While local hosting eliminates many flows, modularity enables all remaining flows to be justified using fine-grained primitives. We introduce two IoT security mechanisms: pipeline permissions that permit device data to be shared given some justification and exit policies that block flows unless specific conditions are met. We evaluate Karl through two end-to-end applications.

==> sections/acknowledgments.tex <==
\section{Acknowledgments}
We thank our shepherd, Michael Ferdman, the anonymous ATC reviewers, and the members of Stanford Future Data for their invaluable feedback on this work.
This research was supported in part by affiliate members and other supporters of the Stanford DAWN project---Ant Financial, Facebook, Google, Infosys, NEC, and VMware---as well as the NSF under CAREER grant CNS-1651570. Any opinions, findings, and conclusions or recommendations expressed in this material are those of the authors and do not necessarily reflect the views of the National Science Foundation.

==> sections/introduction.tex <==
%-------------------------------------------------------------------------------
\section{Introduction}
%-------------------------------------------------------------------------------

The complexity of the modern smart home has made it harder to defend
(Fig.~\ref{fig:overview-ss}).
First, modern devices are tightly integrated with both vendor cloud
services and companion apps, increasing their attack
surface~\cite{alrawi2019sok}.
Second, as these devices
handle more sensitive user data, the potential damage from hackers
and ransomware increases~\cite{ubiquiti2021krebs,roberts2021parler,bitdefender2021ring,sears2019fox,greenberg2018echo,larson2017fda,garlati2016owlet,antonakakis2017understanding,zdnet2021osborne}.
Third, users expect devices from different vendors
to integrate with each other
(e.g., a light and an Alexa
speaker)~\cite{dixon2012operating,smartthings,homekit},
which has led to third-party integrations with over-privileged access.
% for centralized ``hubs".
This complexity is compounded by the heterogeneity in vendors
who manage the devices and cloud infrastructure that need
to access user data~\cite{alrawi2019sok}.
% but can this
% really help once users come to expect a wide variety of services that
% depend on private data sharing and processing?

The reliance on remote hardware has also made it harder for users to
enforce and articulate sensible privacy policies.
Existing mechanisms such as policy legalese and
software configuration boxes, obfuscated by encrypted network traffic, are
impossible to audit once data has been offloaded~\cite{jensen2004privacy,earp2005examining}.
Laws such as GDPR attempt to mandate the safety of cloud
infrastructure~\cite{gdpr,ccpa}, but their efficacy ultimately relies on
vendor expertise.
Centralized ``hubs" enable permission-based access control
between devices from different vendors
and the Internet, but these primitives are too
coarse-grained~\cite{celik2018sensitive,fernandes2016security,lee2017fact,dixon2012operating}.
IoT frameworks need security mechanisms that can express
the privacy guarantees users actually care about.

A more promising approach would be to move the processing and storage
required out of devices and centralized vendor services altogether,
leveraging local hardware.
By shifting all functionality to a locally-hosted hub,
we can reduce the size of the attack surface
and relieve vendors from having to protect millions of users' data.
Also, user-managed hardware gives users more control, allowing them
to express and enforce privacy policies
in terms of fine-grained primitives with semantic meaning
about \textit{why} data is processed, not just who.

% A more promising approach would be to move the processing
% and storage required for IoT devices out of centralized vendor
% services altogether, so that vendors could only be responsible for
% making high-quality hardware and software instead of protecting
% millions of users' data.
% We believe that individual IoT device vendors are unlikely to make
% significant improvements in privacy barring some sort of paradigm shift.
% A smart home is only as secure as its weakest link, and it is
% hard to write secure software for embedded systems with long lifetimes.
% Most vendors don't have the resources to get security right, and the few
% that do also happen to be the companies best placed to monetize private
% user data.  A more promising approach would be to move the processing
% and storage required for IoT devices out of centralized vendor
% services altogether, so that vendors could only be responsible for
% making high-quality hardware and software instead of protecting
% millions of users' data.

\input{figures/overview.tex}

% Smart homes have become attractive targets for hackers and ransomware
% attacks given their easy access to sensitive user
% data~\cite{ransomware,attack,iot,hackers}. In response, legislators attempt
% to require vendors to secure their IoT products based on privacy policies
% such as GDPR\cite{gdpr,ccpa}. However, the heterogeneous IoT industry is
% made up of more than 14.3K unique vendors globally~\cite{kumar2019}, and
% profit is driven by the convenience and functionality a product
% provides~\cite{serena}. Thus in the absence of strict regulation, this
% heterogeneity makes it impossible to ensure that vendors possess both the
% technical expertise and the incentives to comply.

% Centralized IoT hubs can make it easier to protect sensitive user data.
% Existing hubs and research frameworks allow developers to implement
% \textit{apps} or \textit{modules} to integrate their IoT devices with the
% hub. The user can then install these apps to make simple control flow
% decisions and relay commands between devices, such as turning on a light
% when motion is detected. The hub then automatically enforce access control
% and dataflow rules between devices, apps, and the Internet.

% However, the IoT ecosystem includes more than just device logic, and
% existing hubs leak data through these other channels for functionality.
% Specifically, IoT devices must interact with mobile companion apps and
% offload compute to cloud services via the Internet,
% which is outside the scope of frameworks that monitor dataflow up to the network boundary.
% Consider the following: A user checks if a door is locked using a mobile
% app for the smart lock. The lock relays its state to the user through the
% cloud, leaking this information. In another scenario, a user asks a smart
% speaker to turn on a light. The speaker must offload speech-to-text due to
% hardware limitations, but the cloud service may now store the audio, sell
% it to advertisers, or inadvertently leak it in a data breach.
% Thus although existing hubs capture data provenance on local hardware, the
% fate of other sensitive data in the cloud remains unknown.

\input{figures/security_mechanisms.tex}

\input{tables/network_justifications.tex}

In this paper, we present Karl, a new smart home framework that
eliminates dependence on vendor services---prioritizing
privacy through local hosting---while supporting the complex functionality
of modern devices (Fig.~\ref{fig:overview}).
Karl gives devices a simple but expressive programming model with
\textit{modules} that process data, such as speech-to-intent,
and communicate with each other through a key-value \textit{data store}.
% We imagine either vendors or third-party developers to write module software.
The smart home is represented by a dataflow graph,
where device data flows through modules to other devices and the network
(Fig.~\ref{fig:dataflow-graph}).
Users can either interact with the graph directly, or through an automation
frontend.
Each privileged data or network access is validated by a
locally-hosted \textit{Karl hub}.
The hub also serves \textit{Karl apps} that visualize data and
modules, directly to the user's phone.

This programming model applies several features
of the recent serverless paradigm to modern IoT~\cite{jonas2019cloud}:
(1) the disaggregation of storage and compute from the IoT
device allows functionality to exist agnostic of hardware location,
(2) the modularity of the dataflow graph enables fine-grained privacy
policies with semantic meaning, and
(3) the popularity of event-driven programming makes serverless a
familiar interface to developers used to a commercial cloud.

While local hosting eliminates many flows,
modularity enables all remaining flows to be
\textit{justified} using fine-grained primitives.
Karl provides two security mechanisms
(Fig.~\ref{fig:security-mechanisms}):
First, Karl automatically generates easily-reviewable
\emph{pipeline permissions} that describe \textit{why} device data
can flow to another device or the network
(e.g., the speaker must share a location to query the weather).
Second, Karl allows users to set \emph{exit policies} on data
to block flows unless specific conditions based on modules are met
% across all their devices and the network
(e.g., data derived from raw audio can only exit if it
has first been transformed to a textual intent).
Compared to existing IoT frameworks, Karl can provide more ubiquitous and
meaningful privacy guarantees.

Karl tackles four major challenges to achieve its goals of eliminating
dependence on vendor services and enabling expressive privacy policies
on all remaining network accesses:

\paragraph{Supporting Complex Device and Service Interactions}
The first challenge is accounting for the entire attack surface of
modern devices (Table~\ref{tab:class}).
Consider a smart speaker such as the Amazon Alexa or Google Home.
Due to hardware constraints, the speaker must offload some computation
and storage.
When the user interacts with the speaker through a companion app,
they must go through a cloud endpoint mediated by the vendor.
The speaker may also download firmware updates, share analytics,
or otherwise pull and push data to the Internet.
Each network interaction adds a security risk.
% Each network access is another source of risk
%to leak sensitive data.

Existing IoT frameworks were not designed for the network security demands of
modern IoT devices.
Industry hubs like SmartThings~\cite{smartthings}
and research frameworks built on top
of it~\cite{tian2017smartauth,jia2017contexiot}
still require vendors to host their own infrastructure.
For example, Alexa's SmartThings integration serves only to allow
a connection with Amazon servers.
Frameworks like FlowFence~\cite{fernandes2016flowfence} mediate
remote connections through the hub,
but still permit many flows to leak data when not fundamentally required.
For example, FlowFence explicitly allows sharing a door lock's state with the
Internet since it is required for the mobile companion app.

In comparison, Karl moves modern functionality
to trusted hardware under a simple but expressive
programming model,
inspired by the recent popularity of serverless computing.
Karl executes its modules locally and also hosts the data store
on local hardware.
The Karl hub also runs and serves companion apps directly to a user's phone
through a user's router.
% , without requiring data to leave trusted hardware.
Flows that use an external service, such as downloading firmware updates,
can still contact those services but \textit{only if the user allows}
with Karl's security mechanisms.
These basic abstractions enable most device-to-device and companion app
interactions to run on Karl-controlled hardware,
rather than on vendor infrastructure or the IoT devices themselves.

% When functionality cannot be executed on user-owned hardware, the
% home cloud allows users to control when and why their data is shared.
% This access to the Internet is mediated through
% \emph{pipeline permissions}, easily defined by the user in a graphical interface
% and mapped to English-language privacy guarantees.
% Pipeline permissions follow three guiding concepts:
% some modules must be able to access the network, these modules
% should only handle data once it has been transformed a certain way,
% and one instance of a module cannot leak the data of a previous instance.
% % For example, to specify that a security camera
% % can only share analytics if the data has been anonymized,
% % the user requires an anonymization module to process the data
% % before it leaves the home cloud (Fig.~\ref{fig:example}c).
% To enforce pipeline permissions, the home cloud automatically compiles the
% policy graphs down to \textit{tags}, labels that justify the transfer
% of data between and out of sandboxed modules.
% However, there are several challenges to designing a home cloud that
% preserves existing device functionality while protecting user privacy.

% In this paper, we argue that the next smart home framework needs to be based on a single unified programming model that captures the entirety of sensitive data processed by IoT devices.
% We observe that the recent serverless paradigm, as a general-purpose programming model, has the flexibility to capture the three main components of the IoT ecosystem: device-side logic, companion apps, and cloud services.
% We present Karl, a new smart home framework that provides several advantages in security, privacy, and performance unique to the IoT domain as a result of this unified serverless programming model.

\paragraph{Usable Privacy Policies}
The second challenge is expressing privacy policies
when a device \textit{must} access the Internet.
Existing techniques are either obfuscated in cloud infrastructure or based on
coarse-grained security primitives such as device-to-device access control.
In comparison, local hosting enables Karl to enforce ubiquitous policies that
consider all components of modern IoT functionality, as opposed to blindly
trusting multiple vendors.
Modules also enable finer-grained privacy policies with semantic meaning
such as requiring audio data to be converted to text.
Thus Karl's programming model empowers users to express and enforce
privacy policies that correspond to more intuitive privacy guarantees.

We additionally co-design functionality and policies in Karl
such that modifying one reflects in the other. In particular, Karl
enforces user privacy policies by modifying the dataflow graph that
represents device functionality to comply with pipeline permissions
and exit policies, such as by disabling network access or deleting an edge.
Karl treats the generated graph as a
declarative policy, automatically labeling data with non-hierarchical
tags in the data store and enforcing mandatory access control on the
edges.  This mechanism combines the power of information
flow with the simplicity of access control to enforce useful privacy policies
at a fine granularity.

\paragraph{Performance}
A third challenge is maintaining reasonable performance for
real-time user interactions and compute-heavy tasks without
amortizing costs on vendor hardware.
The disaggregation of storage and compute makes it simple for Karl
to be hosted on underutilized hardware the user
already owns, such as an old laptop.
% The Karl hub hosts a data store and executes modules in one or more
% sandboxes on the hub or other user-chosen hardware.
By utilizing local hardware, Karl can minimize latencies for real-time
interactions~\cite{satyanarayanan2017emergence}.
For heavy compute tasks such as ML, which typically run as
stateful services in the cloud, Karl accounts for the
high initialization times of stateless services using our variant of
speculative execution for serverless modules.
%% MZ: commented this out since it doesn't seem that novel and you only have 1 laptop?
%Karl also schedules modules on available hardware
%based on data locality to optimize for performance.
Overall, we find that Karl always has acceptable performance, and
in some cases outperforms cloud services by avoiding the WAN.

\paragraph{System Administration}
Though Karl is best hosted on local hardware
for privacy, end users may prefer the durability and
scalability of the cloud.
% One concern may be that Karl must be on or the smart home loses
% functionality, but that is also the case for a home router or any other
% device that relies on the availability of Internet and electricity.
We show it is feasible to deploy Karl in the cloud but
on \textit{user-managed hardware},
a similar approach to DIY Hosting~\cite{palkar2017diy}.
The cloud deployment increases network latency and costs money,
but self-hosting Karl
in the cloud (e.g., using Amazon Web Services) is still
comparable in cost to popular IoT cloud subscriptions,
and improves privacy because the user need only trust their own
cloud provider rather than vendors and their
providers.\\

%Thus this alternative deployment
%may be suitable for certain users.

% Finally, Karl has the ability to utilize user-managed cloud hardware instead
% of local hardware. While we think it is feasible to have a 24/7 deployment
% at home, such as a router, the cloud allows users to try out the infrastructure
% without committing to hardware maintenance. It comes at the cost of higher
% latency, but scalability may be better.

We implement and evaluate a functioning prototype of Karl.
We port three popular home IoT devices---a security
camera, smart speaker, and light bulb---with privacy concerns due
to their access to sensitive raw data. We implement several applications in
which these devices interact with each other and untrusted third parties
outside the home network.
% Our hub hosts web apps that users can use to remotely monitor their home.
We analyze several privacy expectations that users may
express but cannot be enforced in existing industry hubs and research
systems, and demonstrate how they are intuitive to define
and enforce in Karl. In addition, we demonstrate that Karl offers
reasonable performance and can improve the latency
of some real-time interaction applications.
Finally, we analyze the tradeoffs of self-hosting Karl in the cloud.

In summary, we make the following contributions:
\begin{itemize}

  \item We introduce Karl's modular programming model,
    which makes it practical to support the rich interactions of modern
    devices on local, user-managed hardware.

  \item We introduce \textit{pipeline permissions},
    which restrict devices to justifiable data flows based on
    finer-grained primitives with semantic meaning.
    % \textit{why} data is processed.

  \item We introduce \emph{exit policies} as a way to capture
    end-to-end confidentiality policies users care about and avoid
    unintended consequences of pipeline permissions.

  \item We present and evaluate an implementation of Karl on
    applications spanning 4 devices and 10 modules.

%    We demonstrate that Karl maintains reasonable performance for
%    real-time user interactions and computational tasks on local
%    hardware, and can also be hosted on user-managed cloud hardware at
%    just \$20/month.
\end{itemize}


==> sections/security.tex <==
\section{Security Discussion}
\label{sec:security-analysis}

We analyze the security of Karl first in terms of the features we can
implement in the centralized framework that typically must be
implemented by each vendor, and then by the potential threats imposed
by the design itself.

\subsection{Threat Model}

\subsection{Centralization Advantage}

The unification of the IoT ecosystem under a single expressive framework
enables Karl to address security gaps otherwise plagued by heterogeneity.
Some of these vulnerabilities include insecure discovery and communication
protocols, insecure web admin pages with bad default passwords, and
excessive port forwarding or UPnP.
The best practices to address these problems are built-in to Karl.
In addition, vendors can more easily opt to not host cloud infrastructure
for mediating remote connections, or being liable for managing sensitive
data under strict regulations like GDPR.
The importance of a centralized framework is that it helps vendors focus on
the new functionality they provide rather than the reinventing the
infrastructure to protect user data each time.

\subsection{Hub Security Analysis}

Now we analyze the security of Karl in the context of its new features.
We assume a single user, and trusted
user-owned hardware. We do not trust modules or sensors to exercise
only their assigned privileges. We assume the shared network can contain
passive and active attackers.

Malicious sensors that are paired with the home cloud are limited by
their single network connection to the controller. As long as the
firewall is configured correctly, they cannot directly talk to wide-area
domains or other devices on the network. The sensor could DoS the
controller with data, in which case the controller should rate limit
requests and notify the user. The user can then upgrade their hardware
in the case of normal high traffic, or block the malicious sensor.
Sensors can blast physical information through their actuators to
other devices, but we expect these attacks to be easy to detect.
Sensors may use local communication protocols like Bluetooth and Zigbee,
avoiding the IP router. At the very least, these are pure-local
communication protocols, and shared data must still be transformed
by pipeline permissions.

Malicious modules could have greater impact on user privacy due to the
user's trust in modules to transform data as specified. We believe
that the global module repository should only permit modules that
are open-source to best align with our privacy principles. The modules we
implemented used less than 100 LOC, and some as little as 5, so we
believe they could be easily audited by a technical community.
If the module must be closed-source, the repository could follow a
model similar to app stores where code is vetted by a trusted moderator.
As previously discussed, the host prevents modules from accessing
invalid tags, and the sandbox keeps modules from interfering with the
host machine. The host enforces module timeouts to preserve their
ephemerality. The module repository should also implement a software
update system in case of bugs in module code.

Network attackers can incur the standard attacks of DoSing the network
or inferring information based on network traffic metadata. For these,
we defer to security best practices for quickly detecting network
intrusion. We note that if the user deploys a home cloud where the
controller and host are on the same machine, the passive attacker
has little information about device functionality beyond raw sensor
data and network accesses. An active attacker could impersonate a
sensor or host, which we prevent with standard secure authentication
mechanisms. The webserver's visual secure pairing mechanism provides
another layer of defense against the user approving malicious
participants in the home cloud.

The biggest risk to the home cloud, as with many software systems, is
likely the end user. Thus the home cloud must be easy to setup and
configure, and the visual interface for defining pipeline permissions
must be easy to navigate. For these, we assert that user-focused
software engineering and empirical studies must be performed before
the system is deployed to non-technical users. However, we believe
that the existing heterogeneous state of IoT is already so insecure
that even a misconfigured Karl deployment may be an improvement.


==> sections/threat_model.tex <==
\section{Threat Model}

The parties we consider in our threat model include hardware vendors,
module developers, and Karl users.
Our security goal is to minimize the potential for
sensitive user data to be shared against user expectations.
% who also write device firmware, developers who write module software,
% and users who setup and configure Karl.

Hardware vendors write firmware for the devices they sell.
Malicious firmware can attack the local network,
send data to the Internet, expose ports, or be unintentionally buggy.
Some vendors may host cloud services
that devices contact through modules.
These services can misuse data, or be breached.

Module developers write software to be distributed to users
through a package manager.
Each module is a black-box function and specification that
describes expected inputs, outputs, and network domain names.
Module developers may provide incorrect or overly-permissive
specifications that mislead users.
The software may also try to break out of a sandbox to access
local processes, the filesystem, or the network.

Users set up the Karl hub and configure privacy policies.
The home network may be targeted by common attacks involving
weak credentials, unencrypted traffic, exposed ports, etc.
Misconfigured policies can cause users to leak more data than desired
through Karl or send invalid data to cloud services.
% Users may also try to steal proprietary module software, which runs locally.

% Vendors honest but curious.
% Reputation to protect but monetize data.

% Devices can have software flaws.
% Service can be compromised.
% Zero day stuff, no update.

% Explicitly designed to be familiar.
% List things attackers do that we protect against.

\subsection{Assumptions}
We assume the platform is implemented as described, and
supported similarly to other open-source projects.
The dataflow graph accurately reflects the user's pipeline
permissions and exit policies, and the Karl hub accurately
validates data and network accesses according to the graph.
We assume Karl properly sandboxes module code.
Karl also correctly implements security best practices
including network traffic encryption and multi-factor authentication
for UI access.

We assume that hardware vendors and module developers
are well-intentioned with reputations to uphold.
We thus consider intentional phishing, side channel, and out-of-band
attacks such as communicating with another device through
a physical medium to be egregious and out of scope.

We assume that modules are easily audited against their specifications.
We expect auditing to be performed by a crowdsourced community
or trusted distributor, similar to an app store.
We assume that well-intentioned developers write modules at a
small enough granularity to be tested as black-box functions,
and find this granularity to be practical for a wide number of
applications in our evaluation.
Karl can also log actual module inputs and outputs for
retroactive auditing.

We assume the initial users of Karl to be privacy-conscious
tinkerers who already own multiple connected devices.
We believe these users to be able to configure privacy policies
at the level of a beginner programmer familiar with
block-based languages such as Scratch~\cite{maloney2010scratch},
which uses similar concepts to those in Karl's dataflow graph
and other home automation frameworks such as Home Assistant.

We assume the user correctly configures their router to expose
only the Karl hub to the WAN, and the devices only to the Karl hub.
Note that in the standard IoT model, users may need to expose ports
from individual IoT devices to the WAN, or to each other, which is
less secure.
% Users are expected to restrict their IoT devices to only be able to
% contact the Karl hub on the LAN, as opposed to other devices or the WAN.

% Finally, hackers in our threat model are more incentivized to target
% individual Karl users rather than cloud vendors, since most valuable
% data will be locally-hosted.
% Compared to the standard model, where every IoT device is exposed
% to the Internet and the home network, only the Karl hub is exposed.
% We argue it is more secure for Karl to be implementing best practices
% such as network traffic encryption and multi-factor authentication,
% rather than relying on multiple vendors.

